Learning Gaussian Mixtures Using the Wasserstein-Fisher-Rao Gradient Flow

Gaussian mixture models form a flexible and expressive parametric family of distributions that has found applications in a wide variety of applications. Unfortunately, fitting these models to data is a notoriously hard problem from a computational perspective. Currently, only moment-based methods enjoy theoretical guarantees while likelihood-based methods are dominated by heuristics such as Expectation-Maximization that are known to fail in simple examples. In this work, we propose a new algorithm to compute the nonparametric maximum likelihood estimator (NPMLE) in a Gaussian mixture model. Our method is based on gradient descent over the space of probability measures equipped with the Wasserstein-Fisher-Rao geometry for which we establish convergence guarantees. In practice, it can be approximated using an interacting particle system where the weight and location of particles are updated alternately. We conduct extensive numerical experiments to confirm the effectiveness of the proposed algorithm compared not only to classical benchmarks but also to similar gradient descent algorithms with respect to simpler geometries. In particular, these simulations illustrate the benefit of updating both weight and location of the interacting particles.

==> FRGD.tex <==

\subsection{Fisher-Rao gradient descent \label{subsec:Fisher-Rao-main}}

The Fisher-Rao distance $d_{\mathsf{FR}}(\cdot,\cdot)$ between two
probability measures $\rho_{0},\rho_{1}\in\mathcal{P}(\mathbb{R}^{d})$
is defined as \citep{gallouet2017jko,bauer2016uniqueness}
\begin{align}
d_{\mathsf{FR}}^{2}\left(\rho_{0},\rho_{1}\right) & =\inf\bigg\{\int_{0}^{1}\int\Big[\Big(\alpha_{t}-\int\alpha_{t}\mathrm{d}\rho_{t}\Big)^{2}\Big]\mathrm{d}\rho_{t}\mathrm{d}t:~
\left(\rho_{t},\alpha_{t}\right)_{t\in[0,1]}\,\text{solves}\nonumber \\
 & \qquad\qquad\qquad\partial_{t}\rho_{t}=\rho_{t}\Big(\alpha_{t}-\int\alpha_{t}\mathrm{d}\rho_{t}\Big)\bigg\}.\label{eq:FR-metric}
\end{align}
When $\rho_{0},\rho_{1}\in\mathcal{P}_{\mathrm{ac}}(\mathbb{R}^{d})$,
the Fisher-Rao metric can be expressed as
\[
d_{\mathsf{FR}}^{2}\left(\rho_{0},\rho_{1}\right)=4\int\big|\sqrt{\rho_{0}\left(x\right)}-\sqrt{\rho_{1}\left(x\right)}\big|^{2}\mathrm{d}x,
\]
which is known to statisticians as the squared Hellinger distance
(up to some constant multiple). Equipped with this metric, the Fisher-Rao
gradient flow $\{\rho_{t}\}_{t\geq0}$ of the function $\ell_{N}(\rho)$
is defined by the following PDE:
\begin{equation}
\partial_{t}\rho_{t}=-\left[1+\delta\ell_{N}\left(\rho_{t}\right)\right]\rho_{t}.\label{eq:Fisher-Rao-GF}
\end{equation}
The formal derivation based on Riemannian geometry can be found in
Appendix \ref{subsec:FR-derivation}. By time discretization, one
can also obtain the Fisher-Rao gradient descent updates $\{\rho_{n}\}_{n\geq0}$:
\begin{equation}
\frac{\mathrm{d}\rho_{n+1}}{\mathrm{d}\rho_{n}}=1-\gamma\left[1+\delta\ell_{N}\left(\rho_{n}\right)\right],\qquad n=0,1,\ldots,\label{eq:Fisher-Rao-GD}
\end{equation}
where $\gamma>0$ is the step size. Although Fisher-Rao gradient flow/descent
is derived in an abstract way using Riemannian geometry, it has intimate
connection with some well-known algorithms.
\begin{itemize}
\item {\bf Fisher-Rao gradient flow as proximal gradient flow}. Fisher-Rao
gradient flow \eqref{eq:Fisher-Rao-GF} can be viewed as the continuous-time
limit of the proximal gradient algorithm under the Fisher-Rao metric:
\begin{equation}
\partial_{t}\rho_{t}=\lim_{\eta\to0+}\frac{\rho_{t}^{\eta}-\rho_{t}}{\eta},\quad\text{where}\quad\rho_{t}^{\eta}\coloneqq\underset{\rho\in\mathcal{P}(\mathbb{R}^{d})}{\arg\min}\left\{ \int_{\mathbb{R}^{d}}\delta\ell_{N}\left(\rho_{t}\right)\mathrm{d}\left(\rho-\rho_{t}\right)+\frac{1}{2\eta}d_{\mathsf{FR}}^{2}\left(\rho,\rho_{t}\right)\right\} .\label{eq:FR-proximal}
\end{equation}
\item {\bf Fisher-Rao gradient flow as mirror flow}. The Fisher-Rao gradient flow \eqref{eq:Fisher-Rao-GF} can also be viewed as
the continuous-time limit of mirror descent algorithm for $\ell_{N}(\rho)$
with Kullback-Leibler (KL) divergence
\begin{equation}
\partial_{t}\rho_{t}=\lim_{\eta\to0+}\frac{\rho_{t}^{\eta}-\rho_{t}}{\eta},\quad\text{where}\quad\rho_{t}^{\eta}\coloneqq\underset{\rho\ll\rho_{t}}{\arg\min}\left\{ \int_{\mathbb{R}^{d}}\delta\ell_{N}\left(\rho_{t}\right)\mathrm{d}\left(\rho-\rho_{t}\right)+\frac{1}{\eta}\mathsf{KL}\left(\rho\,\Vert\,\rho_{t}\right)\right\} .\label{eq:FR-mirror}
\end{equation}
\item {\bf Fisher-Rao gradient descent as fixed-location EM algorithm}.
When $\rho_{0}$ is discrete, Fisher-Rao gradient descent \eqref{eq:Fisher-Rao-GD}
with step size $\gamma=1$ coincides with the fixed-location EM algorithm
for Gaussian mixture model in e.g.~\citet{jiang2009general}.
\end{itemize}
Formal justifications of the above three connections can be found
in Appendix \ref{subsec:FR-equivalence}. The below theorem shows
that when $\rho_{0}$ is well-spread,
the Fisher-Rao gradient descent enjoys appealing convergence
property. The proof is deferred to \Cref{sec-convergence-proofs}.

	

\begin{theorem}[Convergence to NPMLE] \label{thm:FR-convergence}
Suppose that the initialization $\rho_{0}\in\mathcal{P} (\mathbb{R}^{d})$ satisfies $\supp (\rho_0) = \RR^d$. Consider the Fisher-Rao gradient descent $\{\rho_{n}\}_{n\geq0}$ defined
in \eqref{eq:Fisher-Rao-GD}. 
There exists $\eta_{0}$ determined by the samples $\{X_{i}\}_{1\leq i\leq N}$, such that if $0<\eta\leq\eta_{0}$ and $\rho_{n}\overset{\mathrm{w}}{\to}\widehat{\rho}$ when $n\to\infty$, then $\widehat{\rho}$ is the NPMLE.
\end{theorem}


The convergence result in Theorem \ref{thm:FR-convergence} is conditional:
we only show that if Fisher-Rao gradient descent converges weakly
to some limiting distribution $\widehat{\rho}$, then $\widehat{\rho}$
is an NPMLE. This is similar to the convergence theory in \citet{chizat2018global},
and is due to a lack of geodesic convexity.
We can also show a similar result for the continuous-time Fisher-Rao gradient flow  $(\rho_{t})_{t\geq0}$ (i.e.~a distributional solution to the PDE \eqref{eq:Fisher-Rao-GF}): if $\rho_{t}\overset{\mathrm{w}}{\to}\widehat{\rho}$ as $t\to\infty$, then $\widehat{\rho}$ is an NPMLE.




\paragraph{Particle Fisher-Rao gradient flow/descent and their inadequacy.}

Theorem \ref{thm:FR-convergence} provides convergence guarantees
for Fisher-Rao gradient flow/descent when initialized from a well-spread distribution. However it is not computationally affordable to implement the dynamic
of a continuous distribution in $\mathbb{R}^{d}$. In practice, we
can only initialize from a discrete distribution with $m$ particles
\[
\rho_{0}=\sum_{l=1}^{m}\omega_{0}^{(l)}\delta_{\mu^{(l)}},\text{ where }\mu^{(1)},\ldots,\mu^{(m)}\in\mathbb{R}^{d}\text{ and }\omega_{0}=(\omega_{0}^{(1)},\ldots,\omega_{0}^{(m)})\in\Delta^{m-1}.
\]
The following theorem characterizes the Fisher-Rao gradient flow when
initialized from a discrete distribution $\rho_{0}$ with $m$ mass
points. 

\begin{theorem}[Particle Fisher-Rao gradient flow]\label{thm:FR-ODE}The
ODE system 
\begin{equation}
\dot{\omega}_{t}^{(j)}=-\omega_{t}^{(j)}\left[1-\frac{1}{N}\sum_{i=1}^{N}\frac{\phi\left(X_{i}-\mu^{(j)}\right)}{\sum_{l=1}^{m}\omega_{t}^{(l)}\phi\left(X_{i}-\mu^{(l)}\right)}\right],\qquad1\leq j\leq m\label{eq:FR-ODE}
\end{equation}
with initialization $\omega_{0}=[\omega_{0}^{(j)}]_{1\leq j\leq m}\in\Delta^{m-1}$
has unique solution on any time interval $[0,T]$. Moreover, the flow
$(\rho_{t})_{t\geq0}$ defined as
\begin{equation}
\rho_{t}\coloneqq\sum_{l=1}^{m}\omega_{t}^{(l)}\delta_{\mu^{(l)}}\label{eq:FR-discrete-solution}
\end{equation}
is the Fisher-Rao gradient flow, i.e.~\eqref{eq:FR-discrete-solution}
is a distributional solution to the PDE \eqref{eq:Fisher-Rao-GF}.

\end{theorem}

The proof is deferred to Appendix \ref{sec:proof-FR-ODE}. In practice,
we can further discretize the gradient flow \eqref{eq:FR-discrete-solution}
and obtain an implementable Fisher-Rao gradient descent algorithm,
which is described in Algorithm \ref{alg:FR-GD}. 

\begin{algorithm}[h]
\caption{Fisher-Rao gradient descent.}

\label{alg:FR-GD}\begin{algorithmic}

\STATE \textbf{{Input}}: data $\{X_{i}\}_{1\leq i\leq n}$, number
of particles $m$, step sizes $\eta>0$, maximum number of iterations
$t_{0}$.

\STATE \textbf{{Initialization}}: draw $\mu^{(1)},\ldots,\mu^{(m)}\overset{\text{i.i.d.}}{\sim}\mathsf{Uniform}(\{X_{i}\}_{1\leq i\leq n})$
and $\omega_{0}^{(1)}=\cdots=\omega_{0}^{(m)}=1/m$.

\vspace{0.2em}

\STATE \textbf{{Updates}}: \textbf{for }$t=0,1,\ldots,t_{0}$ \textbf{do}

\STATE \vspace{-1em}
 \begin{subequations} 
\begin{align*}
\omega_{t+1}^{(j)} & =\omega_{t}^{(j)}+\eta\left[\frac{1}{N}\sum_{i=1}^{N}\frac{\phi\left(X_{i}-\mu^{(j)}\right)}{\sum_{l=1}^{m}\omega_{t}^{(j)}\phi\left(X_{i}-\mu^{(l)}\right)}-1\right]\omega_{t}^{(j)},
\end{align*}
\end{subequations} for all $j=1,\ldots,m$. Here $\phi(x)=(2\pi)^{-d/2}\exp(-\Vert x\Vert_{2}^{2}/2)$
is the probability density function of $\mathcal{N}(0,I_{d})$.

\STATE \textbf{{Output}} $\rho=\sum_{j=1}^{m}\omega_{t_{0}}^{(j)}\delta_{\mu^{(j)}}$
as the (approximate) NMPLE.

\end{algorithmic}
\end{algorithm}

There is a major flaw of this Fisher-Rao gradient flow/descent:
we can see from \eqref{eq:FR-discrete-solution} that the locations
of the particles are fixed at their initialization and only the weights of the particles
are updated. This introduces an approximation error
\[
\min_{\omega\in\Delta^{m-1}}\ell_{N}\left(\sum_{l=1}^{m}\omega^{(l)}\delta_{\mu^{(l)}}\right)-\min_{\rho\in\mathcal{P}(\mathbb{R}^{d})}\ell_{N}\left(\rho\right)
\]
that becomes unavoidable after choosing the initial locations of
the particles \citep{wang2021nonparametric}. A practical scheme is to randomly sample the initial
locations from the sample set $\{X_{i}\}_{1\leq i\leq N}$. Since
the sample data $\{X_{i}\}_{1\leq i\leq N}$ does not necessarily
cover the support of NPMLE \citep{laird1978nonparametric}, it is impossible
for Fisher-Rao gradient flow/descent to converge to the NPMLE. For
example, when the underlying model is a finite-component Gaussian
mixture, the samples are usually not close to the true centers (especially
when the dimension $d$ is high), which leads to non-negligible approximation
error. We will see in Section \ref{sec:numerical} that Fisher-Rao
gradient descent does not perform well in numerical experiments. 

\begin{comment}
$S=\{\mu^{(1)},\ldots,\mu^{(m)}\}\subset\mathbb{R}^{d}$ and consider
only the probability distribution in the probability simplex $\Delta(S)$.
By parameterizing $\rho=\sum_{j=1}^{m}\omega^{(j)}\delta_{\mu^{(j)}}$
for some weight vector $\omega=(\omega^{(1)},\ldots,\omega^{(m)})$
in the standard $(m-1)$-simplex $\Delta^{m-1}$, we can rewrite the
loss function w.r.t.~$\rho$ in \eqref{eq:finite-sample-loss} to
be a loss function w.r.t.~$\omega$: 
\[
f_{m}\left(\omega\right)\coloneqq\ell_{N}\left(\sum_{i=1}^{m}\omega^{(i)}\delta_{\mu^{(i)}}\right)=-\frac{1}{N}\sum_{i=1}^{N}\log\left[\sum_{l=1}^{m}\omega_{l}\phi\left(X_{i}-\mu^{(l)}\right)\right].
\]
The mirror descent algorithm for solving the convex optimization 
\begin{equation}
\underset{\omega\in\Delta^{m-1}}{\arg\min}f_{m}\left(\omega\right)\label{eq:mirror-descent-finite-particle}
\end{equation}
can be described as follows: we first initialize $\omega_{0}\in\Delta^{m-1}$,
then in each iteration $n=0,1,\ldots$ we solve
\[
\omega_{n+1}\coloneqq\arg\min_{\omega\in\Delta^{m-1}}\left\{ f_{m}\left(\omega_{n}\right)+\left\langle \nabla f_{m}\left(\omega_{n}\right),\omega-\omega_{n}\right\rangle +\frac{1}{\eta}D_{\varphi}\left(\omega,\omega_{n}\right)\right\} 
\]
where $D_{\varphi}(x,z)\coloneqq\varphi(x)-\varphi(z)-\langle\nabla\varphi(z),x-z\rangle$
is the Bregman divergence associated with some convex and differentible
function $\varphi$ over $\Delta^{m-1}$. When $\varphi$ is the negative
entropy $\varphi(x)=\sum_{i=1}^{m}x_{i}\log(x_{i})$, then the Bregman
divergence $D_{\varphi}(x,z)$ is the KL divergence $\mathsf{KL}(x\Vert z)=\sum_{l=1}^{m}x_{i}\log(x_{i}/z_{i})$
and we have the following closed-form update rule:
\[
\omega_{n+1}^{(j)}=\frac{\omega_{n}^{(j)}\exp\left(-\eta\left[\nabla f_{m}\left(\omega_{n}\right)\right]_{j}\right)}{\sum_{l=1}^{m}\omega_{n}^{(l)}\exp\left(-\eta\left[\nabla f_{m}\left(\omega_{n}\right)\right]_{l}\right)},\quad\forall\,j\in[m].
\]
Let $\rho_{n}^{(m)}\coloneqq\sum_{l=1}^{m}\omega_{n}^{(l)}\delta_{\mu^{(l)}}$,
we can compute
\[
\left[\nabla f_{m}\left(\omega_{n}\right)\right]_{j}=-\frac{1}{N}\sum_{i=1}^{N}\frac{\phi\left(X_{i}-\mu^{(j)}\right)}{\sum_{l=1}^{m}\omega_{n}^{(l)}\phi\left(X_{i}-\mu^{(l)}\right)}=-\frac{1}{N}\sum_{i=1}^{N}\frac{\phi\left(X_{i}-\mu^{(j)}\right)}{\rho_{n}^{(m)}*\phi\left(X_{i}\right)}=\delta\ell_{N}\left(\rho_{n}^{(m)}\right)(\mu^{(j)}),
\]
we know that as $\eta\to0$, for all $j\in[m]$
\begin{align*}
\omega_{n+1}^{(j)} & =\omega_{n}^{(j)}\frac{1-\eta\left[\nabla f_{m}\left(\omega_{n}\right)\right]_{j}+O(\eta^{2})}{\sum_{l=1}^{m}\omega_{t}^{(l)}\left\{ 1-\eta\left[\nabla f_{m}\left(\omega_{n}\right)\right]_{l}\right\} +O(\eta^{2})}=\omega_{n}^{(j)}\frac{1-\eta\delta\ell_{N}\left(\rho_{n}^{(m)}\right)(\mu^{(j)})+O(\eta^{2})}{1-\eta_{t}\sum_{l=1}^{m}\omega_{n}^{(l)}\delta\ell_{N}\left(\rho_{n}^{(m)}\right)(\mu^{(j)})+O(\eta^{2})}\\
 & =\omega_{n}^{(j)}\frac{1-\eta\delta\ell_{N}\left(\rho_{n}^{(m)}\right)(\mu^{(j)})+O(\eta^{2})}{1+\eta+O(\eta^{2})}=\omega_{n}^{(j)}\frac{\left[1-\eta\delta\ell_{N}\left(\rho_{n}^{(m)}\right)(\mu^{(j)})+O(\eta^{2})\right]\left(1-\eta\right)}{1+O(\eta^{2})}\\
 & =\omega_{n}^{(j)}\left\{ 1-\eta\left[1+\delta\ell_{N}\left(\rho_{n}^{(m)}\right)(\mu^{(j)})\right]+O(\eta^{2})\right\} .
\end{align*}
\end{comment}



==> WassersteinGD.tex <==
\subsection{Wasserstein gradient descent \label{subsec:Wasserstein-main}}

The empirical and theoretical advantage of Wasserstein-Fisher-Rao
gradient descent/flow over Fisher-Rao counterpart raises a natural
question: is Wasserstein gradient update  \eqref{eq:WFR-GD-W} alone
adequate for computing NPMLE? Although we have achieved some preliminary results, a complete answer to that
question is still not clear. In this section we briefly introduce the Wasserstein gradient
flow/descent for NPMLE, and defer the theoretical properties and discussions to Appendix
\ref{sec:Wass-theory}. 

Given two probability measures $\rho_{0},\rho_{1}\in\mathcal{P}(\mathbb{R}^{d})$,
the quadratic Wasserstein distance between $\rho_{0}$ and $\rho_{1}$
is defined as \citep{villani2009optimal}
\[
d_{\mathsf{W}}^{2}\left(\rho_{0},\rho_{1}\right)=\inf_{\pi\in\Pi(\rho_{0},\rho_{1})}\int\left\Vert x-y\right\Vert _{2}^{2}\pi\left(\mathrm{d}x,\mathrm{d}y\right),
\]
where the infinium is taken over all coupling of of $\rho_{0}$ and
$\rho_{1}$. From the perspective of Riemannian geometry, it also admits
the following expression
\begin{align}
d_{\mathsf{W}}^{2}\left(\rho_{0},\rho_{1}\right) & =\inf\bigg\{\int_{0}^{1}\int\left\Vert v_{t}\right\Vert ^{2}\mathrm{d}\rho_{t}\mathrm{d}t:\left(\rho_{t},v_{t}\right)_{t\in[0,1]}\;\text{solves}\;\partial_{t}\rho_{t}=-\mathsf{div}\left(\rho_{t}v_{t}\right)\bigg\}.\label{eq:Wass-metric}
\end{align}
In Appendix \ref{subsec:Wass-derivation} we derive the gradient flow
of $\ell_{N}(\rho)$ under the Wasserstein geometry, which evolves
according to the PDE
\begin{equation}
\partial_{t}\rho_{t}=\mathsf{div}\left(\rho_{t}\nabla\delta\ell_{N}\left(\rho_{t}\right)\right)\label{eq:Wass-GF}
\end{equation}
The corresponding discrete time algorithm is
\[
\rho_{t+1}=\left[\mathrm{id}-\eta\nabla\delta\ell_{N}\left(\rho_{t}\right)\right]_{\#}\rho_{t},\qquad t=0,1,\ldots
\]
for some step size $\eta>0$. When initialized from a discrete distribution
\[
\rho_{0}=\frac{1}{m}\sum_{l=1}^{m}\delta_{\mu_{0}^{(l)}},\text{ where }\mu_{0}^{(1)},\ldots,\mu_{0}^{(m)}\in\mathbb{R}^{d},
\]
the following theorem gives a concise characterization of the Wasserstein
gradient flow. The proof can be found in Appendix \ref{sec:proof-Wass-ODE}.

\begin{theorem}[Particle Wasserstein gradient flow]\label{thm:Wass-ODE}The
ODE system 
\begin{align}
\dot{\mu}_{t}^{(j)} & =\frac{1}{N}\sum_{i=1}^{N}\frac{\phi\left(X_{i}-\mu_{t}^{(j)}\right)}{\sum_{l=1}^{m}\omega_{t}^{(j)}\phi\left(X_{i}-\mu_{t}^{(l)}\right)}\left(X_{i}-\mu_{t}^{(j)}\right),\label{eq:Wass-ODE}
\end{align}
with initialization $\mu_{0}^{(1)},\ldots\mu_{0}^{(m)}\overset{\text{i.i.d.}}{\sim}\mathsf{Uniform}(\{X_{i}\}_{1\leq i\leq N})$
has unique solution on any time interval $[0,T]$. Moreover, the flow
$(\rho_{t})_{t\geq0}$ defined as
\begin{equation}
\rho_{t}\coloneqq\frac{1}{m}\sum_{l=1}^{m}\delta_{\mu_{t}^{(l)}}\label{eq:Wass-discrete}
\end{equation}
is the Wasserstein gradient flow, i.e.~ \eqref{eq:Wass-discrete}
is a distributional solution to the PDE  \eqref{eq:Wass-GF}.

\end{theorem}

By time discretization, we also have the Wasserstein gradient descent
algorithm; see Algorithm \ref{alg:Wasserstein-GD}. 
\begin{algorithm}[h]
\caption{Wasserstein gradient descent.}

\label{alg:Wasserstein-GD}\begin{algorithmic}

\STATE \textbf{{Input}}: data $\{X_{i}\}_{1\leq i\leq n}$, number
of particles $m$, step sizes $\eta>0$, maximum number of iterations
$t_{0}$.

\STATE \textbf{{Initialization}}: draw $\mu_{0}^{(1)},\ldots,\mu_{0}^{(m)}\overset{\text{i.i.d.}}{\sim}\mathsf{Unif}(\{X_{i}\}_{1\leq i\leq n})$.

\vspace{0.2em}

\STATE \textbf{{Updates}}: \textbf{for }$t=0,1,\ldots,t_{0}$ \textbf{do}

\STATE \vspace{-1em}
 \begin{subequations} 
\begin{align*}
\mu_{t+1}^{(j)} & =\mu_{t}^{(j)}+\eta\frac{1}{N}\sum_{i=1}^{N}\frac{\phi\left(X_{i}-\mu_{t}^{(j)}\right)}{m^{-1}\sum_{l=1}^{m}\phi\left(X_{i}-\mu_{t}^{(l)}\right)}\left(X_{i}-\mu_{t}^{(j)}\right),
\end{align*}
\end{subequations} for all $j=1,\ldots,m$. Here $\phi(x)=(2\pi)^{-d/2}\exp(-\Vert x\Vert_{2}^{2}/2)$
is the probability density function of $\mathcal{N}(0,I_{d})$.

\STATE \textbf{{Output}} $\rho=m^{-1}\sum_{j=1}^{m}\delta_{\mu_{t_{0}}^{(j)}}$
as the (approximate) NMPLE.

\end{algorithmic}
\end{algorithm}

Similar to Fisher-Rao gradient descent/flow, the fact that Wasserstein
gradient flow/descent does not update the weight of the particles
also introduces the following approximation error that becomes unavoidable
after choosing the number of particles $m$:
\[
\min_{\mu_{1}\ldots,\mu_{m}\in\mathbb{R}^{d}}\ell_{N}\left(\frac{1}{m}\sum_{l=1}^{m}\delta_{\mu_{l}}\right)-\min_{\rho\in\mathcal{P}(\mathbb{R}^{d})}\ell_{N}\left(\rho\right).
\]
We can minimize this approximation error by choosing a sufficiently
large $m$. In fact, we can check that the ODE system  \eqref{eq:Wass-ODE}
that captures the dynamic of Wasserstein gradient flow  \eqref{eq:Wass-discrete}
is equivalent to the Euclidean gradient flow for the following overparameterized
MLE 
\begin{equation}
\argmin_{\mu_{1}\ldots,\mu_{m}\in\mathbb{R}^{d}}
\ell\left(\mu_{1},\ldots,\mu_{m}\right)=-\frac{1}{N}\sum_{i=1}^{N}\log\left[ \frac{1}{m}\sum_{j=1}^{m}\phi\left( X_{i}-\mu_{j}\right)\right] ,\label{eq:overparameterized-likelihood}
\end{equation}
and the update rule of the location of particles in Algorithm \ref{alg:Wasserstein-GD}
is the Euclidean gradient descent for  \eqref{eq:overparameterized-likelihood}. 

\paragraph{Summary}

\begin{table}
\caption{Gradient flows of $\ell_{N}$ over $\mathcal{P}(\mathbb{R}^{d})$
w.r.t.~different metrics.\label{table:algorithms}}

\centering

\begin{tabular}{|c|c|c|}
\hline 
Riemannian metric & Gradient flow & Particle gradient descent\tabularnewline
\hline 
Fisher-Rao  \eqref{eq:FR-metric} & $\partial_{t}\rho_{t}=-\left[1+\delta\ell_{N}\left(\rho_{t}\right)\right]\rho_{t}$ & Algorithm \ref{alg:FR-GD}\tabularnewline
\hline 
Wasserstein-Fisher-Rao  \eqref{eq:WFR-metric} & $\partial_{t}\rho_{t}=\mathsf{div}\left(\rho_{t}\nabla\delta\ell_{N}\left(\rho_{t}\right)\right)-\left[1+\delta\ell_{N}\left(\rho_{t}\right)\right]\rho_{t}$ & Algorithm \ref{alg:WFR-GD}\tabularnewline
\hline 
Wasserstein  \eqref{eq:Wass-metric} & $\partial_{t}\rho_{t}=\mathsf{div}\left(\rho_{t}\nabla\delta\ell_{N}\left(\rho_{t}\right)\right)$ & Algorithm \ref{alg:Wasserstein-GD}\tabularnewline
\hline 
\end{tabular}
\end{table}

In this section we have introduced three gradient flow/descent algorithms
for the loss function $\ell_{N}(\rho)$ under different Riemannian
structures, which are summarized in Table \ref{table:algorithms}.
When initialized from a distribution spread out over the whole space,
both Fisher-Rao and Wasserstein-Fisher-Rao gradient descent/flow enjoy
nice convergence properties. However in practice when we are only
able to track the dynamic of gradient flow/descent from a discrete
initial distribution, Wasserstein-Fisher-Rao gradient descent is our
algorithm of choice, due to its capability of changing the weight
and the location of the particles simultaneously in each iteration.
In Section \ref{sec:numerical} we will conduct a series of numerical
experiments to compare these three algorithms. As we will see momentarily,
Wasserstein-Fisher-Rao gradient descent achieves the best performance
in all experimental settings. 


==> prior_art.tex <==

\section{Additional related literature}

\paragraph{Structural results of NPMLE.}

The structure of NPMLE for Gaussian mixture in one dimension has been
extensively studied in prior literature. Classical results in \citet{laird1978nonparametric,lindsay1983bgeometry,lindsay1983ageometry,groeneboom1992information,lindsay1993uniqueness}
show that when the sample size is $N$, NPMLE is unique and is a discrete
distribution with at most $N$ atoms. Although this upper bound is
tight in general, in practice the support size is usually much smaller.
The recent work \citep{polyanskiy2020self} show that the support size
of NPMLE is upper bounded by $O((X_{\max}-X_{\min})^{2})$ where $X_{\max}$
(resp.~$X_{\min}$) is the largest (resp.~smallest) sample. When
the mixing distribution $\rho^{\star}$ is sub-Gaussian, this upper
bound suggests that with high probability NPMLE is $O(\log N)$-atomic.
To the best of our knowledge, there is no known structural result
for NPMLE in higher dimension. 

\paragraph{Statistical properties of NPMLE.}

The consistency of NPMLE for Gaussian mixture is studied in \citet{kiefer1956consistency}.
In terms of estimation accuracy, \citet{zhang2009generalized,dicker2016high,saha2020nonparametric}
provide the upper bound on the squared Hellinger distance between
$\widehat{\rho}*\mathcal{N}(0,1)$ and $\rho^{\star}*\mathcal{N}(0,1)$
in one dimension, and \citet{polyanskiy2020self} claims that the proof
in these papers can be extended to higher dimension, which leads to
the bound $O((\log n)^{d+1}/n)$ when the dimension $d$ is a constant.
The accuracy of NPMLE for estimating the mixing distribution in Gaussian
mixture is not studied in prior literature, although \citet{miao2021fisher}
provide estimation error bound in Wasserstein-$1$ distance in the
context of Poisson mixture.

\paragraph{Wasserstein-Fisher-Rao gradient flow.}

Wasserstein-Fisher-Rao distance is defined in \citet{chizat2018interpolating,kondratyev2016new,liero2018optimal}
as an interpolating distance between Wasserstein \citep{villani2009optimal}
and Fisher-Rao distance \citep{bauer2016uniqueness}. The distance
is closely related to unbalanced optimal transport \citep{chizat2018unbalanced}.
There has been a few papers that use Wasserstein-Fisher-Rao gradient
flow to study problems in statistics and machine learning. For example,
it is used in \citet{lu2019accelerating,lu2022birth} to accelerate the mixing
of Langevin diffusion in sampling multimodal distribution, is used
in \citet{lambert2022variational} to design algorithms for variational
inference, and is also used in \citet{rotskoff2019global} to accelerate
the training of two-layer neural networks. In addition, although Wasserstein
gradient descent/flow is not the algorithm of choice in the current
paper, prior literature that uses Wasserstein gradient flow to study
neural network in the mean-field regime, e.g.~\citet{chizat2018global,mei2018mean,sirignano2020mean}
is also related to this paper. We refer the readers to \citet{ambrosio2008gradient,santambrogio2017euclidean}
for a systematic tutorial on Wasserstein gradient flow, and \citet{gallouet2017jko}
for more discussion on Fisher-Rao and Wasserstein-Fisher-Rao gradient
flow.

